Clustering Residential Electricity Consumption Data to Create Archetypes that Capture Household Behaviour in South Africa

Clustering is frequently used in the energy domain to identify dominant electricity consumption patterns of households, which can be used to construct customer archetypes for long term energy planning. Selecting a useful set of clusters however requires extensive experimentation and domain knowledge. While internal clustering validation measures are well established in the electricity domain, they are limited for selecting useful clusters. Based on an application case study in South Africa, we present an approach for formalising implicit expert knowledge as external evaluation measures to create customer archetypes that capture variability in residential electricity consumption behaviour. By combining internal and external validation measures in a structured manner, we were able to evaluate clustering structures based on the utility they present for our application. We validate the selected clusters in a use case where we successfully reconstruct customer archetypes previously developed by experts. Our approach shows promise for transparent and repeatable cluster ranking and selection by data scientists, even if they have limited domain knowledge.

==> sections/Notes.tex <==
section 2:
alluded to the fact that kmeans & som are clear winners, even though they aren't really
the conclusion should be that they are widely used, not that they are the best

keep a note of all the things I change and then highlight them in a revised pdf

we needed to create archetypes for SA, and this was a method for solving it locally

we framed the paper as a method, even though it's a actually a case study for an approach that could turn into a method. To fix this I need to:
adapt title
adapt introduction
adapt discussion
adapt conclusion
